Interactive-Rate Supervisory Control for Arbitrarily-Routed Multi-Tendon Robots via Motion Planning

Tendon-driven robots, where one or more tendons under tension bend and manipulate a flexible backbone, can improve minimally invasive surgeries involving difficult-to-reach regions in the human body. Planning motions safely within constrained anatomical environments requires accuracy and efficiency in shape estimation and collision checking. Tendon robots that employ arbitrarily-routed tendons can achieve complex and interesting shapes, enabling them to travel to difficult-to-reach anatomical regions. Arbitrarily-routed tendon-driven robots have unintuitive nonlinear kinematics. Therefore, we envision clinicians leveraging an assistive interactive-rate motion planner to automatically generate collision-free trajectories to clinician-specified destinations during minimally-invasive surgical procedures. Standard motion-planning techniques cannot achieve interactive-rate motion planning with the current expensive tendon robot kinematic models. In this work, we present a 3-phase motion-planning system for arbitrarily-routed tendon-driven robots with a Precompute phase, a Load phase, and a Supervisory Control phase. Our system achieves an interactive rate by developing a fast kinematic model (over 1,000 times faster than current models), a fast voxel collision method (27.6 times faster than standard methods), and leveraging a precomputed roadmap of the entire robot workspace with pre-voxelized vertices and edges. In simulated experiments, we show that our motion-planning method achieves high tip-position accuracy and generates plans at 14.8 Hz on average in a segmented collapsed lung pleural space anatomical environment. Our results show that our method is 17,700 times faster than popular off-the-shelf motion planning algorithms with standard FK and collision detection approaches. Our open-source code is available online.

==> Makefile <==
TOPLEVEL     := tendon-motion-planning.tex
TARGET       := tendon-motion-planning.pdf
DIFF_TARGET  := diff.pdf
ZIP_TARGET   := $(TOPLEVEL:%.tex=%.zip)
DRAFT_TARGET := $(TARGET:%.pdf=%-draft.pdf)
TARGETS      := $(TARGET)
TARGETS      += $(DIFF_TARGET)
COPY_TARGETS := $(TARGETS:%.pdf=%-copy.pdf)
GREY_TARGETS := $(TARGETS:%.pdf=%-grey.pdf)
ZIP_DIR      := $(basename $(ZIP_TARGET))
MAKEFILES    := Makefile
MAKEFILES    += color_out.mk

DEPFILES     :=
DEPFILES     += $(wildcard *.png)
DEPFILES     += $(wildcard *.cls)
DEPFILES     += $(wildcard inputs/*.tex)
DEPFILES     += $(wildcard inputs/algorithms/*.tex)
DEPFILES     += $(wildcard inputs/figures/*.tex)
DEPFILES     += $(wildcard inputs/tables/*.tex)
DEPFILES     += $(wildcard inputs/notes/*.tex)
DEPFILES     += $(wildcard *.bib)
DEPFILES     += $(wildcard images/*.pdf)
DEPFILES     += $(wildcard images/*.png)
DEPFILES     += $(wildcard images/in-progress/*.pdf)
DEPFILES     += $(wildcard images/timing/*.pdf)
DEPFILES     += $(TOPLEVEL)

ZIPFILES     :=
ZIPFILES     += $(MAKEFILES)
ZIPFILES     += $(TOPLEVEL)
ZIPFILES     += Logo.png
ZIPFILES     += bullet.png
ZIPFILES     += ieeeaccess.cls
ZIPFILES     += images/bentl.jpg
ZIPFILES     += images/bentl1.pdf
ZIPFILES     += images/bentl10.pdf
ZIPFILES     += images/bentl11.pdf
ZIPFILES     += images/bentl2.jpg
ZIPFILES     += images/bentl3.pdf
ZIPFILES     += images/bentl4.png
ZIPFILES     += images/bentl5.pdf
ZIPFILES     += images/bentl6.pdf
ZIPFILES     += images/bentl7.pdf
ZIPFILES     += images/bentl8.pdf
ZIPFILES     += images/bentl9.pdf
ZIPFILES     += images/kuntz.jpg
ZIPFILES     += images/rucke.jpg
ZIPFILES     += inputs/alg-normal-ik.tex
ZIPFILES     += inputs/alg-roadmap-ik.tex
ZIPFILES     += inputs/alg-supervisory-control.tex
ZIPFILES     += inputs/alg-voxelize-free-edge.tex
ZIPFILES     += inputs/apdx-dyn-edge-discretizer.tex
ZIPFILES     += inputs/apdx-fk-solvers.tex
ZIPFILES     += inputs/apdx-ik.tex
ZIPFILES     += inputs/apdx-spherical-sampling.tex
ZIPFILES     += inputs/fig-chosen-lung-points.tex
ZIPFILES     += inputs/fig-collision-compare-config.tex
ZIPFILES     += inputs/fig-collision-compare-edge.tex
ZIPFILES     += inputs/fig-comparison-25-and-200.tex
ZIPFILES     += inputs/fig-config-sampling.tex
ZIPFILES     += inputs/fig-ct-slices.tex
ZIPFILES     += inputs/fig-fig1.tex
ZIPFILES     += inputs/fig-fk-implementations.tex
ZIPFILES     += inputs/fig-milestone-timing-compare-lineplot.tex
ZIPFILES     += inputs/fig-slow-comparison-25.tex
ZIPFILES     += inputs/fig-tendon-robot.tex
ZIPFILES     += inputs/hdr-abstract.tex
ZIPFILES     += inputs/hdr-authors.tex
ZIPFILES     += inputs/hdr-keywords.tex
ZIPFILES     += inputs/hdr-newcommands.tex
ZIPFILES     += inputs/hdr-usepackage.tex
ZIPFILES     += inputs/sec-acknowledgments.tex
ZIPFILES     += inputs/sec-conclusion.tex
ZIPFILES     += inputs/sec-evaluation.tex
ZIPFILES     += inputs/sec-intro.tex
ZIPFILES     += inputs/sec-limitations.tex
ZIPFILES     += inputs/sec-method.tex
ZIPFILES     += inputs/sec-problemdef.tex
ZIPFILES     += inputs/sec-relatedwork.tex
ZIPFILES     += inputs/tail-biography.tex
ZIPFILES     += inputs/tbl-ablation-5000.tex
ZIPFILES     += notaglineLogo.png
ZIPFILES     += tendon-motion-planning.bbl
ZIPFILES     += references.bib

GARBAGE      :=
GARBAGE      += comment.cut
GARBAGE      += $(TOPLEVEL:%.tex=%.log)
GARBAGE      += $(TOPLEVEL:%.tex=%.out)
GARBAGE      += $(TOPLEVEL:%.tex=%.aux)
GARBAGE      += $(TOPLEVEL:%.tex=%.dvi)
GARBAGE      += $(TOPLEVEL:%.tex=%.cb)
GARBAGE      += $(TOPLEVEL:%.tex=%.cb2)
GARBAGE      += $(TOPLEVEL:%.tex=%.bbl)
GARBAGE      += $(TOPLEVEL:%.tex=%.blg)
GARBAGE      += $(TOPLEVEL:%.tex=%.tdo)
GARBAGE      += $(TOPLEVEL:%.tex=%.markdown.in)
GARBAGE      += $(TOPLEVEL:%.tex=%.markdown.lua)
GARBAGE      += $(TOPLEVEL:%.tex=%.markdown.out)
GARBAGE      += $(addprefix _markdown_,$(TOPLEVEL:%.tex=%))
GARBAGE      += $(addprefix _minted-,$(TOPLEVEL:%.tex=%))
GARBAGE      += $(wildcard figures/*-eps-converted-to.pdf)

#TEXPATH      ?= .:inputs:

# To use custom fonts, build with xelatex instead
#LATEX        := TEXINPUTS=$(TEXPATH) pdflatex
LATEX         := pdflatex
LATEX         += -shell-escape
#LATEX         = xelatex
LATEXDRAFT    := $(LATEX) -draftmode
#LATEXDIFF    := TEXINPUTS=$(TEXPATH) latexdiff
LATEXDIFF     := latexdiff
#LATEXDIFF    += --exclude-textcmd="section,subsection"
LATEXPAND     := latexpand

-include color_out.mk

ifndef VERBOSE
.SILENT:
endif

.PHONY: default
default: $(TARGET) $(TARGET:%.pdf=%-copy.pdf) # $(TARGET:%.pdf=%-grey.pdf)

.PHONY: all
all: $(TARGETS) $(COPY_TARGETS) $(GREY_TARGETS) $(ZIP_TARGET)

.PHONY: zip arxiv
zip: $(ZIP_TARGET)
arxiv: zip

.PHONY: draft
draft: $(DRAFT_TARGET)

$(TARGET): $(MAKEFILES) $(DEPFILES)

# print statistics of a tex file compilation
# @param $1: name of the log file
define TEX_STATS
	echo
	$(call bold_color,BLUE,$1 statistics:)
	echo "    ----"
	if grep "^mytodo" $1 >/dev/null; then \
	  $(call color_out_noline,RED,  unaddressed todos:      ); \
	else \
	  $(call color_out_noline,BLUE,  unaddressed todos:      ); \
	fi
	grep "^mytodo" $1 | wc -l
	echo "    ----"
	$(call color_out_noline,BLUE,  overfull:               )
	grep "^Overfull" $1 | wc -l
	$(call color_out_noline,BLUE,  underfull:              )
	grep "^Underfull" $1 | wc -l
	echo "    ----"
	$(call color_out_noline,BLUE,  total warnings:         )
	grep -i warning $1 | wc -l
	$(call color_out_noline,BLUE,  undefined citations:    )
	grep "Warning: Citation .* undefined" $1 | wc -l
	$(call color_out_noline,BLUE,  undefined references:   )
	grep "Warning: Reference .* undefined" $1 | wc -l
	$(call color_out_noline,BLUE,  duplicate labels:       )
	grep "Warning: Label .* multiply defined" $1 | wc -l
	echo "    ----"
	#if [ "$$(type -P detex)" ]; then \
	#	$(call color_out_noline,BLUE,  total word count:       ); \
	#	detex $(1:%.log=%.tex) | wc -w; \
	#  echo "    ----"; \
	#fi
	$(call color_out_noline,BLUE,  pages:                  )
	grep "[0-9]\+ page" $1 | sed -e 's/.*(\([0-9]\+\) page.*/\1/g'
	echo "    ----"
	echo
endef

%-draft.pdf: %.tex $(MAKEFILES) $(DEPFILES)
	@$(call color_out,GREEN,$< -> $@)
	mkdir -p draft
	$(LATEX) -output-directory draft $< </dev/null >/dev/null \
		|| (tail -n 30 $*.log && false)
	-bibtex draft/$*  </dev/null >/dev/null
	cp draft/$*.pdf $@


%.pdf: %.tex $(MAKEFILES)
	@$(call color_out,GREEN,$< -> $@)
	$(LATEXDRAFT) $< </dev/null >/dev/null || (tail -n 30 $*.log && false)
	-bibtex $*  </dev/null >/dev/null
	$(LATEXDRAFT) $< </dev/null >/dev/null
	$(LATEX) $< </dev/null >/dev/null
	$(call TEX_STATS,$*.log)

%-copy.pdf: %.pdf
	@$(call color_out,GREEN,$< -> $@)
	cp $< $@

%-grey.pdf: %.pdf
	@$(call color_out,GREEN,$< -> $@)
	gs \
	  -sOutputFile="$@" \
	  -sDEVICE=pdfwrite \
	  -sColorConversionStrategy=Gray \
	  -dProcessColorModel=/DeviceGray \
	  -dCompatibilityLevel=1.4 \
	  -dNOPAUSE \
	  -dBATCH \
	  -q \
	  "$<"

images/%.eps: images/%.dot
	@$(call color_out,GREEN,$< -> $@)
	dot $< -Tps -o $@

images/%.ps: images/%.tex
	@$(call color_out,GREEN,$< -> $@)
	(cd images && $(LATEX) $(notdir $<)) </dev/null >/dev/null \
		|| (tail -n 30 $(<:%.tex=%.log) && false)

.PHONY: diff
diff: diff.pdf

diff.tex: old.tex new.tex
	@$(call color_out,GREEN,old.tex + new.tex -> $@)
	$(LATEXDIFF) old.tex new.tex 2>/dev/null > diff.tex

new.tex: $(MAKEFILES) $(DEPFILES)
	@$(call color_out,GREEN,$(TOPLEVEL) -> new.tex)
	TEXINPUTS=".:inputs/:" $(LATEXPAND) --fatal --verbose --output new.tex $(TOPLEVEL) 2>/dev/null

GARBAGE    += new.tex
GARBAGE    += diff.tex
TARGETS    += diff.pdf
GARBAGE    += old.log
GARBAGE    += old.out
GARBAGE    += old.aux
GARBAGE    += old.dvi
GARBAGE    += old.cb
GARBAGE    += old.cb2
GARBAGE    += old.bbl
GARBAGE    += old.blg
GARBAGE    += old.tdo
GARBAGE    += old.markdown.in
GARBAGE    += old.markdown.lua
GARBAGE    += old.markdown.out
GARBAGE    += old.pdf
GARBAGE    += new.log
GARBAGE    += new.out
GARBAGE    += new.aux
GARBAGE    += new.dvi
GARBAGE    += new.cb
GARBAGE    += new.cb2
GARBAGE    += new.bbl
GARBAGE    += new.blg
GARBAGE    += new.tdo
GARBAGE    += new.markdown.in
GARBAGE    += new.markdown.lua
GARBAGE    += new.markdown.out
GARBAGE    += new.pdf
GARBAGE    += new.tex
GARBAGE    += diff.log
GARBAGE    += diff.out
GARBAGE    += diff.aux
GARBAGE    += diff.dvi
GARBAGE    += diff.cb
GARBAGE    += diff.cb2
GARBAGE    += diff.bbl
GARBAGE    += diff.blg
GARBAGE    += diff.tdo
GARBAGE    += diff.markdown.in
GARBAGE    += diff.markdown.lua
GARBAGE    += diff.markdown.out
GARBAGE    += diff.tex
GARBAGE    += draft

.PHONY: clean
clean:
	rm -rf $(GARBAGE)

.PHONY: veryclean
veryclean: clean
	rm -f $(TARGETS)
	rm -f $(DRAFT_TARGET)
	rm -f $(COPY_TARGETS)
	rm -f $(GREY_TARGETS)
	rm -rf $(ZIP_DIR)
	rm -f $(ZIP_TARGET)

.PHONY: distclean
distclean: veryclean

$(ZIP_DIR):
	@mkdir -p $(ZIP_DIR)

# @param 1: source file
# @param 2: destination directory
define COPY_TO_PATH
	mkdir -p $(strip $2)/$(strip $(dir $1))
	cp $1 $2/$1
	
endef

$(ZIP_TARGET): $(ZIPFILES) | $(ZIP_DIR)
	@echo "copying files into $(ZIP_DIR)/"
	@$(foreach f,$(ZIPFILES),$(call COPY_TO_PATH,$f,$(ZIP_DIR)))
	@echo "$(ZIP_DIR)/* -> $(ZIP_TARGET)"
	@zip -r $(ZIP_TARGET) $(ZIP_DIR) >/dev/null

